Making Science Simple: Corpora for the Lay Summarisation of Scientific Literature

Lay summarisation aims to jointly summarise and simplify a given text, thus making its content more comprehensible to non-experts. Automatic approaches for lay summarisation can provide significant value in broadening access to scientific literature, enabling a greater degree of both interdisciplinary knowledge sharing and public understanding when it comes to research findings. However, current corpora for this task are limited in their size and scope, hindering the development of broadly applicable data-driven approaches. Aiming to rectify these issues, we present two novel lay summarisation datasets, PLOS (large-scale) and eLife (medium-scale), each of which contains biomedical journal articles alongside expert-written lay summaries. We provide a thorough characterisation of our lay summaries, highlighting differing levels of readability and abstractiveness between datasets that can be leveraged to support the needs of different applications. Finally, we benchmark our datasets using mainstream summarisation approaches and perform a manual evaluation with domain experts, demonstrating their utility and casting light on the key challenges of this task.

==> sections/5.experiments-original.tex <==
\section{Experiments and Results}

We provide benchmark results for our datasets using popular heuristics-based, unsupervised, and supervised summarisation approaches, providing baselines for future works (\S\ref{subsec:results-baselines}). Additionally, we also include results for several additional models which make use of additional data (\S\ref{subsec:results-additional}).

\begin{table*}[ht]
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{llccccccccccc}
        \hline \multirow{2}{*}{\textbf{Approach}} && \multicolumn{5}{c}{\textbf{PLOS}} && \multicolumn{5}{c}{\textbf{eLife}}  \\ \cline{3-7} \cline{9-13}
        & & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{FKGL} & \textbf{DCSR}  && \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{FKGL} & \textbf{DCSR}  \\
        \hline
           \parbox[t]{1mm}{\scriptsize \multirow{4}{*}{\rotatebox[origin=c]{90}{Heuristic}}} 
           \hspace{3pt} \textsc{Lead-3}      && 25.46 & 6.35  & 22.89 & 15.08 & 12.66 && 17.93 & 3.66 & 16.45 & 13.30 & 12.65  \\
           \hspace{8pt} \textsc{Lead-K}      && 35.50 & 8.69  & 32.33 & 14.94 & 11.88 && 34.12 & 6.73 & 32.06 & 11.89 & 10.58 \\
           \hspace{8pt} \textsc{Abstract}    && 47.07 & 18.60 & 43.51 & 14.98 & 11.10 && 28.92 & 6.19 & 27.04 & 15.35 & 11.87 \\ 
           \hspace{8pt} \textsc{Oracle\_Ext} && 56.43 & 31.24 & 52.88 & 15.28 & 11.20 && 46.38 & 11.48 & 43.82 & 13.18 & 10.51 \\ \hline
           \parbox[t]{1mm}{\scriptsize \multirow{4}{*}{\rotatebox[origin=c]{90}{Unsupervised}}}
            \hspace{3pt} \textsc{LSA} && 35.14 & 6.92 & 31.46 & 17.39 & 12.41 && 34.57 & 5.69 & 32.27 & 16.50 & 11.52 \\            
           \hspace{8pt} \textsc{LexRank}  && 36.53 & 9.43 & 33.09 & 14.90 & 10.51 && 30.32 & 5.29 & 28.40 & 13.45 & 9.75  \\
           \hspace{8pt} \textsc{TextRank}  && 36.03 & 8.71 & 32.04 & 20.42 & 11.83 && 31.45 & 5.28  & 29.22 & 19.13 & 11.28 \\
           \hspace{8pt} \textsc{HipoRank}  && 42.16 & 11.41 & 38.01 & 14.91 & 11.82 && 29.95 & 5.38 & 27.44 & 13.58 & 12.32 \\ \hline
           \parbox[t]{1mm}{\scriptsize \multirow{3}{*}{\rotatebox[origin=c]{90}{Supervised}}} 
          \hspace{3pt} \textsc{Pointer-Gen}  &&  &  &  & & &&  &  &  & & \\
           \hspace{8pt} \textsc{Bart}  && 42.35 & 12.96 & 38.57 & 14.62 & 12.07  && 46.57 & 11.65 & 43.70 & 10.94 & 9.36  \\
          \hspace{8pt} \textsc{BigBird}  && 32.76 & 5.11 & 30.21 & 12.58 & 10.63 && 37.03 & 5.71 & 34.89 & 10.62 & 9.55  \\
          \cdashline{1-13}[1.5pt/2pt]
            \hspace{8pt} \textsc{Bart$_{PubMed}$}  && 42.12 & 12.70 & 38.34 & 14.75 & 12.09 && 46.20 & 11.36 & 43.21 & 11.24 & 9.64 \\
           \hspace{8pt} \textsc{Bart$_{Cross}$}  && 42.24 & 13.52 & 38.63 & 14.24 & 12.18  &&  46.22 & 11.53 & 43.33 & 10.81 & 9.31 \\
           \hspace{8pt} \textsc{Bart$_{Scaffold}$}  && 39.47 & 9.73 & 35.79 & 14.45 & 11.74 && 45.28 & 10.99 & 42.51 & 10.65 & 9.19 \\ 
        %   \hspace{8pt} \textsc{Bart$_{Unlikelihood}$} &&  & &  &&  & & \\ 
           \hline
    \end{tabular}
    }
    \caption{Results of summarisation models on our datasets (\textbf{R} = average ROUGE F1-score).}
    \label{tab:summ_results}
\end{table*}

% \begin{table*}[ht]
%     \centering
%     \resizebox{1.0\textwidth}{!}{
%     \begin{tabular}{llccccccccccc}
%         \hline \multirow{2}{*}{\textbf{Approach}} && \multicolumn{5}{c}{\textbf{\textsc{PLOS}}} && \multicolumn{5}{c}{\textbf{\textsc{eLife}}}  \\ \cline{3-7} \cline{9-13}
%         & & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{FKGL} & \textbf{DCSR}  && \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{FKGL} & \textbf{DCSR}  \\
%         \hline
%           \parbox[t]{1mm}{\scriptsize \multirow{4}{*}{\rotatebox[origin=c]{90}{Heuristic}}} 
%           \hspace{3pt} \textsc{Lead-3}      && 25.46 & 6.35  & 22.89 & 15.08 & 12.66 && 18.32 & 3.91 & 16.78 & 13.37 & 12.66 \\
%           \hspace{8pt} \textsc{Lead-K}      && 35.50 & 8.69  & 32.33 & 14.94 & 11.88 && 34.14 & 6.68 & 32.07 & 11.73 & 10.59 \\
%           \hspace{8pt} \textsc{Abstract}    && 47.07 & 18.60 & 43.51 & 14.98 & 11.10 && 29.45 & 6.47 & 27.56 & 15.70 & 11.71 \\ 
%           \hspace{8pt} \textsc{Oracle\_Ext} && 56.43 & 31.24 & 52.88 & 15.28 & 11.20 && 46.43 & 11.76 & 43.95 & 13.52 & 10.55 \\ \hline
%           \parbox[t]{1mm}{\scriptsize \multirow{4}{*}{\rotatebox[origin=c]{90}{Unsupervised}}}
%             \hspace{3pt} \textsc{LSA} && 35.14 & 6.92 & 31.46 & 17.39 & 12.41 && 34.73 & 5.75 & 32.40 & 16.50 & 11.57 \\            
%           \hspace{8pt} \textsc{LexRank}  && 36.53 & 9.43 & 33.09 & 14.90 & 10.51 && 30.60 & 5.72 & 28.80 & 13.65 & 9.76 \\
%           \hspace{8pt} \textsc{TextRank}  && 36.03 & 8.71 & 32.04 & 20.42 & 11.83 && 31.92 & 5.67 & 29.61 & 19.58 & 11.21 \\
%           \hspace{8pt} \textsc{HipoRank}  && 42.16 & 11.41 & 38.01 & 14.91 & 11.82 && 30.34 & 5.58 & 28.00 & 13.87 & 12.45 \\ \hline
%           \parbox[t]{1mm}{\scriptsize \multirow{3}{*}{\rotatebox[origin=c]{90}{Supervised}}} 
%           \hspace{3pt} \textsc{Pointer-Gen}  &&  &  &  & & &&  &  &  & & \\
%           \hspace{8pt} \textsc{Bart}  && 42.35 & 12.96 & 38.57 & 14.62 & 12.07  && 48.72 & 15.76 & 45.95 & 11.17 & 9.61 \\
%           \hspace{8pt} \textsc{BigBird}  && 32.76 & 5.11 & 30.21 & 12.58 & 10.63 && 36.77 & 5.97 & 34.74 & 10.76 & 9.40 \\
%         %   \hspace{8pt} \textsc{BigBird$_{PubMed}$}  &&  & &  &&  & & \\ 
%           \cdashline{1-13}[1.5pt/2pt]
%             \hspace{8pt} \textsc{Bart$_{PubMed}$}  && 42.12 & 12.70 & 38.34 & 14.75 & 12.09 && 49.02 & 15.66 & 46.24 & 11.13 & 9.65 \\
%           \hspace{8pt} \textsc{Bart$_{Cross}$}  && 42.24 & 13.52 & 38.63 & 14.24 & 12.18  && 49.03 & 15.64 & 46.19  & 11.29 & 9.63 \\
%           \hspace{8pt} \textsc{Bart$_{Scaffold}$}  && 39.47 & 9.73 & 35.79 & 14.45 & 11.74  && 47.64 & 14.54 & 44.97 & 11.23 & 9.62 \\ 
%         %   \hspace{8pt} \textsc{Bart$_{Unlikelihood}$} &&  & &  &&  & & \\ 
%           \hline
%     \end{tabular}
%     }
%     \caption{Results of summarisation models on our datasets (\textbf{R} = average ROUGE F1-score).}
%     \label{tab:summ_results}
% \end{table*}



\subsection{Baseline Approaches} \label{subsec:results-baselines}
For our heuristics-based approaches we include the widely-used \textsc{Lead-3} baseline, making use of the first three sentences of the main body of the text. As our lay summaries typically consist of more than three sentences, we also include \textsc{Lead-k} which uses the first $k$ sentences, with $k$ being equal to the average lay summary length for each dataset (Table \ref{tab:datasets}). Additionally, we include the scores obtained by the technical abstracts (\textsc{Abstract}), as well as a greedy extractive \textsc{Oracle}.
% Comment on performance + maybe rephrase above

We benchmark three unsupervised extractive approaches:  \textsc{LexRank} \citep{Erkan_2004}, \textsc{TextRank} \citep{mihalcea-tarau-2004-textrank}, and \textsc{HipoRank} \citep{Dong2021-yh}.

For supervised models, we train and evaluate abstractive transformer-based models, \textsc{BART} \citep{lewis-etal-2020-bart} and \textsc{BigBird} \citep{zaheer2020}.\footnote{We truncate the input to 1024 tokens for \textsc{BART} and 4096 tokens for \textsc{BigBird}.} 
% need to mention any truncation/input reduction (BART max len=1024, bigbird=4096)

\subsection{Additional approaches} \label{subsec:results-additional}
Here, we aim to establish how the use of additional data in various forms can benefit model performance for lay summarisation. To do this, we test the performance of three additional version of \textsc{BART}. 

\paragraph{PubMed pretraining} As our datasets remain smaller than those used for scientific summarisation, we include the results of a version pretrained on the PubMed dataset \citep{Cohan2018-nq} and fine-tuned on our own datasets. This model is denoted by \textsc{BART}$_{PubMed}$.
% mention that both are biomedical domain

\paragraph{Cross pretraining}  
Aiming to assess the how well models trained on our own datasets are able to generalise to the other, we also include version of \textsc{BART} which is pretrained on opposite dataset to that which it is fine-tuned and evaluated on. 
This model is denoted by \textsc{BART}$_{Cross}$. 

\paragraph{Scaffolding}
We also experiment with artificially increasing our dataset size by way of a scaffold task. Inspired by CATTS \citep{Cachola2020-bx}, we remove the article's abstract from the input text and train the model to also generate the abstract as a scaffold task to lay summary generation. In addition to assessing whether training for abstract generation can assist lay summary generation, results for this model will provide an indication of the baseline \textsc{BART} model's reliance on the abstract content.

Specifically, we include two copies of every article within our training data with one using the abstract as reference summary and the other, the lay summary. We distinguish between the two the by prepending the input document with the control tokens \texttt{$\langle|$ABSTRACT$|\rangle$} or \texttt{$\langle|$SUMMARY$|\rangle$}. Documents within the validation and test splits are then prepended the \texttt{$\langle|$SUMMARY$|\rangle$} code to induce lay summary generation. This model is denoted by \textsc{BART}$_{Scaffold}$. 

\subsection{Discussion}
Table \ref{tab:summ_results} presents the performance of the aforementioned approaches on both the PLOS and eLife datasets using automatic metrics. In line with common practice for summarisation, we report the F1-scores of ROUGE-1, 2, and L \citep{lin-2004-rouge}. Additionally, we include FKGL and DCRS scores (see \S\ref{subsec:analysis-readability}) of the generated output, providing an assessment of the syntactic and lexical complexity, respectively. From the results presented, we can draw several conclusions about our datasets.

\paragraph{The importance of the abstract}
Based on the ROUGE scores obtained by the \textsc{Abstract} baseline, we can safely assume that the lay summaries within PLOS are much closer in resemblance to their respective technical abstracts than the lay summaries within eLife. The importance of the abstract in the generation of the lay summary is  highlighted by the performance of the \textsc{BART}$_{Scaffold}$ model, which performs significantly worse than the standard \textsc{BART} model on PLOS, likely due to the removal of the abstract from the model input.  % also a small performance decrease for eLife 

\paragraph{Extractive vs abstractive}
In general, we would expect abstractive methods to have greater application for the task of lay summarisation due to their ability to transform (and thus, simplify) text from the input article. However, state-of-the-art abstractive approaches have a tendency to generate hallucinations, resulting in factual inconsistencies between the source and output \citep{Maynez2020-xd}. Therefore, extractive approaches may still have utility for the task going forward, especially if the comprehensibility of selected sentences is directly considered. 

Of the two datasets, we find the unsupervised extractive baselines perform significantly better on PLOS in terms of ROUGE scores, aligning with observations from our analysis of abstractiveness (\S\ref{subsec:analysis-abstractiveness}). 
% even given this analysis, it is surprising that the ROGUE scores for abstractive models on eLife are as good as they are   

% - Abstractive methods perform better on eLife, and are able to achieve greater ROUGE scores overall for this dataset. Additionally, there is a very large disparity between extractive and abstractive performance on this dataset

% Readability metrics do not seem overly affected by the level of 


% - Extractive methods perform better on PLOS, which makes sense as this is a less abstractive dataset

\paragraph{Use of additional data}
% - Inclusion of PubMed pretraining gives an increase to performance for eLife (the smaller dataset), but not for PLOS (indicating this is large enough to effectively train the model without additional pretraining)
Interestingly, we find that pretraining \textsc{BART} on Pubmed does very little to affect the performance. For both datasets, we actually observe a very slight degradation over the non-pretrained \textsc{BART}, suggesting that habits learnt for abstract generation do not transfer well do lay summarisation.
As previously mentioned, artificially creating more data via an abstract-generation scaffold task also results in a decrease in ROUGE scores for both datasets, indicating a reliance on the abstract content for lay summarisation.  

% Cross training
Similarly, \textsc{BART}$_{Cross}$ achieves a performance similar to that of the non-pretrained model.
% maybe due to differing levels of simplicity

% - Scaffold task does not provide benefit for either dataset, indicating a reliance on abstract content in the generation of a lay summary (already slightly covered).



\subsection{Human evaluation}
To further assess the usability of the generated summaries, we perform an additional human evaluation of our `strongest' baseline model - \textsc{Bart} - using two domain experts.\footnote{Both judges have experience in scientific research and hold at least a bachelor's degree in Biomedical science.} 

The evaluation is carried out using a random sample of 10 articles from the test split of each dataset. Alongside each model-generated summary, judges are presented with both the abstract and reference lay summary of the given article and, using a 1-5 Likert scale, are asked to assess the model output on the following three criteria:
1) \textit{Comprehensiveness} - to what extent does the model output contain all information that might be necessary for a non-expert to understand the high-level topic of the article and the significance of the research;
2) \textit{Layness} - to what extent is the content of the model output comprehensible (or readable) to a non-expert, in terms of both structure and language;
3) \textit{Factuality} - to what extent is the model output factually consistent with the two other provided summaries.
We choose to provide the judges with only this information, rather than the full article text, in an effort to minimise the overall complexity of the evaluation and the cognitive burden placed upon participants.

\begin{table}[]
    \centering
    \begin{tabular}{cccc}
         \hline
         \textbf{Dataset} & \textbf{Comp.} & \textbf{Layness} &\textbf{Factuality} \\ \hline
         PLOS & 3.7 & 3.0 & 3.0 \\
         eLife & 3.1 & 3.0 & 3.0 \\ \hline 
    \end{tabular}
    \caption{Mean evaluator ratings (1-5) obtained by \textsc{Bart} outputs for each metric.}
    \label{tab:human_eval}
\end{table}

Table \ref{tab:human_eval} presents the average ratings from our manual evaluation. We calculate Krippendorff's $\alpha$ to measure inter-rater reliability, where we obtain values of 0.78 and 0.54 for PLOS and eLife, respectively. In addition to providing rating, evaluators also provided comments on the general performance on each criteria for both datasets, providing further insights into model performance.
%% Observations %%

\paragraph{Comprehensiveness}
% Comprehensiveness
% - PLOS does better in this metric, but we can understand from annotator comments that is largely due to heavy use of the abstract.
% - eLife, used less abstract content, but also statements which potentially confusing to the reader (i.e., off topic) - The model seems to start off by introducing the topic well but struggles to hit the \"what is the significance of this research?\" question.

We can see from Table \ref{tab:human_eval} that model output on PLOS is judged to be more comprehensive than on eLife. From evaluator comments, we understand that this largely results from extensive use of abstract content for PLOS, which is sometimes copied directly (or with minor edits) to the lay summary.  
For eLife, it was observed that new information (i.e., not contained in the reference abstract or lay summary) was often introduced which was irrelevant or confusing, potentially affecting the understanding of a lay reader.
% indicating that the model learnt to use focus largely on this part  

\paragraph{Layness}
Interestingly, given the previously highlighted differences in simplicity level between the lay summaries, the average layness of the model output is judged to be equal for both datasets. 
However, evaluator comments indicate that outputs were typically penalised for different reasons for each dataset. For PLOS, the aforementioned heavy use of abstract content often resulted in the inclusion of jargon terms that a lay reader which struggle to interpret. Alternatively, language within eLife outputs was observed to be better suited to a lay audience, but was sometimes simplified to a point that it could be misconstrued and mislead a lay reader, occasionally containing grammatical errors, typos, and repeated content. 

% Layness
% - Interestingly, both datasets obtain the same mean rating for this metric. However, comments reveal this is likely for different reasons. 
% PLOS - heavy use of abstract content resulted in the inclusion of quite a lot of jargon (e.g. Genus species nomenclature) and less background information. 
% - for eLife, the language was much more suited to a lay audience, although jargon was still sometimes present. At times the information was simplified to a point where it could be misconstrued or mislead a lay audience. There were a few grammatical errors and poor sentence structure, typos, repetition etc. 


\paragraph{Factuality}

Again, we find equal average score of 3.0 given for for factuality, suggesting the model struggles to produce factually correct outputs for both datasets. In fact, we found no output from either dataset was given a perfect score by both annotators, indicating that simplifying technical content accurately is a consistent problem. Evaluator comments highlight contradictions, unclear phrasing, and misrepresentation of entities as key contributing factors to factual inconsistencies. We regard this is an integral obstacle to overcome in the development of usable lay summarisation models and an essential focus for future research.

% Factuality
% - Score is again equal, and suggests that there the model struggles to produce a factually consistent output for both datasets. In fact, we found no instance in either dataset was given a perfect score by both annotators, indicating that simplifying technical content accurately is a consistent problem. Comments highlight occasional contradictions, unclear phrasing and 
% - 


% Overall, this evaluation has shed light on the key challenges facing the 

% - Could maybe look at alignment between automatic metrics and ratings for each criteria?

% - Comments




